Towards Egocentric 3D Hand Pose Estimation in Unseen Domains

We present V-HPOT, a novel approach for improving the cross-domain performance of 3D hand pose estimation from egocentric images across diverse, unseen domains. State-of-the-art methods demonstrate strong performance when trained and tested within the same domain. However, they struggle to generalise to new environments due to limited training data and depth perception -- overfitting to specific camera intrinsics. Our method addresses this by estimating keypoint z-coordinates in a virtual camera space, normalised by focal length and image size, enabling camera-agnostic depth prediction. We further leverage this invariance to camera intrinsics to propose a self-supervised test-time optimisation strategy that refines the model's depth perception during inference. This is achieved by applying a 3D consistency loss between predicted and in-space scale-transformed hand poses, allowing the model to adapt to target domain characteristics without requiring ground truth annotations. V-HPOT significantly improves 3D hand pose estimation performance in cross-domain scenarios, achieving a 71% reduction in mean pose error on the H2O dataset and a 41% reduction on the AssemblyHands dataset. Compared to state-of-the-art methods, V-HPOT outperforms all single-stage approaches across all datasets and competes closely with two-stage methods, despite needing approximately x3.5 to x14 less data.

==> tables/TTT_table.tex <==
\begin{table*}[h!]
    \centering
    \caption{3D MPJPE in camera space [mm]. The lower row shows the percentage improvement (\%) in \textcolor{darkgreen}{dark green} (lower is better).}
    \label{tab:datasets}
    \begin{tabular}{lccccc}
        \toprule
        \textbf{Method} & \textbf{Training Data} & \textbf{H2O} & \textbf{FPHA} & \textbf{AssemblyHands} & \textbf{HOT3D} \\
        \midrule
        Baseline & HOT3D & 143.38 & 221.1 & 306.8 & 29.5 \\
        TTT & HOT3D & 51.43 & 93.3 & 176.1 & - \\
        \midrule
        \textbf{Improvement} &  & \textcolor{darkgreen}{\textbf{64.1\%}} & \textcolor{darkgreen}{\textbf{57.8\%}} & \textcolor{darkgreen}{\textbf{42.6\%}} & - \\
        \bottomrule
    \end{tabular}
\end{table*}

==> tables/gt_depth.tex <==
{
\setlength{\tabcolsep}{0.5pt}
\begin{table}[t]
    \centering
    \small
   \caption{\textbf{Impact of depth estimation quality on pose estimation performance.} Comparison between ground truth sensor-based depth and \textit{DPT-Hybrid} pseudo-depth across \textit{HOT3D} and \textit{AssemblyHands} datasets.}
    \label{tab:depth_comparison}
    \begin{tabularx}{\linewidth}{l>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering\arraybackslash}X}
        \toprule
        & \multicolumn{2}{c}{{MPJPE} $\downarrow$} & \multicolumn{2}{c}{{MPJPE-RA} $\downarrow$} & \multicolumn{2}{c}{{MRRPE} $\downarrow$} & \multicolumn{2}{c}{{L2} $\downarrow$} \\
        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}
        \cmidrule(lr){6-7}
        \cmidrule(lr){8-9}
        & HOT & AsHa & HOT & AsHa & HOT & AsHa & HOT & AsHa \\
        \midrule
        \multicolumn{9}{c}{base model} \\
        \midrule
        \textit{GT depth} & 252.9 & 288.6 & 76.9 & 102.7 & 182.8 & 280.6 &15.8 & 59.6 \\
        \textit{DPT-Hyb.} & 250.8 & 289.1 & 75.5 & 100.1 & 180.7 & 276.1 & 16.1 & 57.0 \\
        \midrule
        \multicolumn{9}{c}{V-HPOT} \\
        \midrule        
        
        \textit{GT depth} & 263.2 & 250.7 & 76.9 & 110.6 & 185.0 & 342.1 & 13.0 & 65.9 \\
        \textit{DPT-Hyb.} & 262.6 & 238.8 & 79.7 & 121.5 & 180.2 & 360.1 & 15.7 & 63.2 \\
        \bottomrule
    \end{tabularx}
\end{table}
}
